Probabilistically Robust Learning: Balancing Average- and Worst-case Performance

Many of the successes of machine learning are based on minimizing an averaged loss function. However, it is well-known that this paradigm suffers from robustness issues that hinder its applicability in safety-critical domains. These issues are often addressed by training against worst-case perturbations of data, a technique known as adversarial training. Although empirically effective, adversarial training can be overly conservative, leading to unfavorable trade-offs between nominal performance and robustness. To this end, in this paper we propose a framework called probabilistic robustness that bridges the gap between the accurate, yet brittle average case and the robust, yet conservative worst case by enforcing robustness to most rather than to all perturbations. From a theoretical point of view, this framework overcomes the trade-offs between the performance and the sample-complexity of worst-case and average-case learning. From a practical point of view, we propose a novel algorithm based on risk-aware optimization that effectively balances average- and worst-case performance at a considerably lower computational cost relative to adversarial training. Our results on MNIST, CIFAR-10, and SVHN illustrate the advantages of this framework on the spectrum from average- to worst-case robustness.

==> contents/duality.tex <==
\section{A dual perspective on~\eqref{eq:p-cvar}}

As discussed in the previous section, the optimization problem in~\eqref{eq:p-cvar} and the equivalent formulation in~\eqref{eq:unconst-cvar} are of fundamental interest because (a) they represent the tightest convex relaxation of the constraints in~\eqref{eq:p-const}, (b) they provide a framework where the parameter $\beta\in[0,1]$ links the average- and worst-case problems of~\eqref{eq:p-avg} and~\eqref{eq:p-rob}, and (c) the formulation in~\eqref{eq:unconst-cvar} is unconstrained, and therefore amenable to gradient-based optimization.  However, before we exploit the properties of CVaR toward deriving an algorithm for solving~\eqref{eq:unconst-cvar}, we first study the duality properties of the constrained formulation in~\eqref{eq:p-cvar}.  

To begin, we note that because~\eqref{eq:p-cvar} is \emph{piecewise linear} in the optimization variable $t$,~\eqref{eq:p-cvar} can be directly recharacterized via Lagrangian duality.  Indeed, the following theorem shows that a (strongly) dual counterpart can be obtained for~\eqref{eq:p-cvar}.
%
\begin{theorem} \label{thm:dual-cvar}
If the map $(x,y)\mapsto \ell(f_\theta(x),y)\in L^p$ for $p\in(1,\infty)$, then~\eqref{eq:p-cvar} is equivalent to
%
\begin{align}
    \min_{\theta\in\Theta} \max_{\nu\in\calP^q(\beta)} \E_{(x,y)} \E_{\delta\sim\nu(\delta|x,y)} \left[\ell(f_\theta(x+\delta),y) \Prob_\Delta(\delta) \right] \label{eq:cvar-dual}
\end{align}
%
Here $q$ satisfies $(1/p) + (1/q) = 1$ and $\calP^q(\beta)\subset L^q$ contains the elements $\nu\in L^q$ satisfying (a) $\nu(\delta|x,y) \in [0, 1/\beta]$ almost everywhere, (b) $\nu(\delta|x,y)$ is absolutely continuous with respect to $\Prob$ and $\Prob_\Delta$, and (c) $\nu(\delta|x,y)$ is normalized along $\Delta$, i.e. $\int_\Delta \nu(\delta|x,y)\Prob_\Delta(\delta)\text{d}\delta = 1$ for a.e.\ $x,y\in \Omega$.
\end{theorem}
%
Concretely, this problem shows that~\eqref{eq:p-cvar} is equivalent to a distributionally robust optimization (DRO) problem over perturbation distributions.  In particular, the inner maximization in~\eqref{eq:cvar-dual} involves optimizing over conditional measures $\nu(\delta|x,y)$ that can place mass at most $1/\beta$ on any particular perturbation $\delta\in\Delta$.   Notably, this result can also be seen as a lifting of the finite-dimensional, nonlinear problem of computing CVaR in~\eqref{eq:unconst-cvar} to an infinite-dimensional, \emph{linear} optimization problem.

The proof of this theorem relies on the strong duality of linear programs and the Radon-Nikodym theorem to rewrite the problem in terms of the dual variables $\nu(\delta|x,y)$ for each $(x,y)\in\Omega$.  Indeed, this result generalizes the well-known dual characterization of CVaR~\cite{rockafellar2000optimization} in that the measure $\nu(\delta|x,y)$ in the inner maximization is required to be absolutely continuous with respect to both $\Prob_\Delta$ and $\Prob$.  For details, see Appendix~\textcolor{red}{X}.

\paragraph{Characterizing the optimal distribution $\nu^\star(\delta|x,y)$.}  Despite the convexity of CVaR, computing the optimal thresholding variables $\alpha$ in~\eqref{eq:def-cvar} can be time consuming for high-dimensional distributions $\Prob_\Delta$.  To this end, one notable feature of the dual problem derived in Theorem~\ref{thm:dual-cvar} is that under fairly general conditions, the inner maximization problem admits a~\emph{closed-form} solution.  In the following theorem, we use variational duality theory to fully characterize this optimal perturbation distribution $\nu^\star(\delta|x,y)$.

\begin{theorem} \label{thm:opt-dual-dist}
In the setting of Thm.~\ref{thm:dual-cvar}, if $p=q=2$, then for each $(x,y)\in\Omega$, there exists constants $\gamma(x,y)>0$ and $\mu(x,y)\in\R$ such that
%
\begin{align}
    \nu^\star(\delta|x,y) = \min\left\{ \left( \frac{\ell(f_\theta(x+\delta),y) - \mu(x,y)}{\gamma(x,y)}\right)_+, \frac{1}{\beta}\right\} \notag
\end{align}
%
is the solution to the inner maximization over measures $\nu\in\calP^2(\beta)$.  Moreover, the values of $\mu$ and $\gamma$ are such that
%
\begin{align}
    \int_\Delta \Pi_{[0,1/\beta]} \left\{ \frac{\ell(f_\theta(x+\delta),y) - \mu(x,y)}{\gamma(x,y)} \right\} \text{d}\delta = 1
\end{align}
%
for all $(x,y)\in\Omega$, where $\Pi_{[0,1/\beta]}$ denotes the projection onto the interval $[0,1/\beta]$.
\end{theorem}

This theorem shows that the optimal distribution is characterized by a truncated version of the loss of the classifier, where the truncation is applied below at zero and above at $1/\beta$.  Notably, the fact that the optimal distribution can place mass no larger than $1/\beta$ on any given perturbation precludes the possibility of $\nu^\star(\delta|x,y)$ being a Dirac distribution, as is the case in the worst-case optimization problem~\eqref{eq:p-rob}, which can be seen as placing mass only on those examples $\delta^\star$ satisfying $\delta^\star\in\argmax_{\delta\in\Delta} \ell(f_\theta(x+\delta),y)$.

\paragraph{Statistical learning through~\eqref{eq:cvar-dual}.}  Although in general for $\beta>0$ it is an open problem regarding how one can sample from the optimal distribution $\nu^\star$, this optimal distribution can be fully characterized in special cases.  Of particular interest is 

\begin{proposition}
Under the conditions of Theorem~\ref{thm:opt-dual-dist}, let us additionally assume that $\Delta$ is compact and that $\ell$ is the 0-1 loss.  Then the optimal distribution $\nu^\star(\delta|x,y)$ is given by
%
\begin{align}
    \nu^\star(\delta|x,y) = \begin{cases}
        \min\left\{\frac{1}{m_\textup{err}}, \frac{1}{\beta}\right\} \quad\quad \textup{if } f_\theta(x+\delta) \neq y \\
        \frac{1}{1 - m_\textup{err}}\left(1 - \min\left\{1, \frac{m_\textup{err}}{\beta}\right\}\right)\quad \textup{otherwise.} 
    \end{cases} \notag
\end{align}
%
where $m_\textup{err} = \Prob_\Delta\{f_\theta(x+\delta)\neq y\}$.
\end{proposition}

\paragraph{Sample complexity}


==> old/abstract.tex <==
\begin{abstract}
Many of the successes of deep learning are based on minimizing a cost function on average.  However, it is well-known that this paradigm suffers from a lack of adversarial robustness, which hinders its applicability in safety-critical domains.  This issue is often addressed by training against worst-case perturbations of data, a technique known as adversarial training.    Although empirically effective, adversarial training can be unnecessarily conservative and is known to suffer from trade-offs between nominal performance and robustness.  To this end, we propose a framework called probabilistic robustness to bridge the gap between the accurate, yet brittle average case and the robust, yet conservative worst case by enforcing robustness to most rather than to all perturbations.  From a theoretical point of view, this framework overcomes certain trade-offs between robust and nominal performance in high dimensions.  Moreover, it avoids the pathological behaviors associated with the learning complexity of adversarial training.  From a practical point of view, its connections to risk-aware estimation provide an effective algorithm, whose performance on standard benchmarks illustrates the advantages of balancing the average case and the worst case.

% putting forward a high-probability counterpart of robustness which interpolates that 
\end{abstract}

==> old/formulation.tex <==
\section{Probabilistic robustness}

As discussed in the previous section, the learning community is in need of an principled and interpretable robustness framework that interpolates between the average and worst-case.  Furthermore, given the limitations of previous frameworks, it is essential that any candidate robust learning paradigm should admit a tractable algorithmic framework.  To this end, in this section, we propose a new framework, which we call \emph{probabilistic robustness}, to fill this gap.

\paragraph{A probabilisitc view of robustness.}

The basis for our framework takes root in recent work that has sought to explain the practical and theoretical barriers inherent to robust learning in the sense of~\eqref{eq:p-rob}.  In this body of work, several recent papers have argued that adversarial examples lie on a lower-dimensional manifold in the data space~\cite{gilmer2018adversarial,khoury2018geometry,shamir2021dimpled}. \hh{this is good motivation--can you write it in a way that you don't need the word ``manifold". No problem if not. Also, can you check if Zico's original smoothing paper has the same observation?} This suggests that in order to solve~\eqref{eq:p-rob}, one must search over regions of the data space that have extremely low probability, resulting in the empirically-observed conservatism of adversarially-trained classifiers.  Given this perspective, our approach will be to introduce a probabilistic framework for robustness in which robustness is enforced to most rather than to all perturbations.

To embed this idea into a concrete formulation for robust learning,  following~\cite{robey2021adversarial} our starting point is to observe that~\eqref{eq:p-rob} can be equivalently rewritten as the following semi-infinite \emph{constrained} optimization problem
%
\begin{alignat}{2}
    &\min_{\theta\in\Theta, \: t\in L^p} &&\E_{(x,y)} t(x,y) \tag{P-EPI} \label{eq:p-epi}\\
    &\st &&[\ell(f_\theta(x+\delta),y)] \leq t(x,y) \quad\forall (x,y,\delta) \notag
\end{alignat}
%
by using an epigraph formulation for the inner maximization problem in the objective of~\eqref{eq:p-rob}.  The equivalence of these two problems follows directly from the fact that for each instance-label pair $(x,y)\in\Omega$, the inequality $\max_{\delta\in\Delta} \ell(f_\theta(x+\delta),y) \leq t(x,y)$ holds if and only if the inequality $\ell(f_\theta(x+\delta),y) \leq t(x,y)$ holds for every $\delta\in\Delta$.  Note that in this formulation, we have introduced a (functional) optimization variable $t\in L^p(\Omega, \calB, \Prob)$ that, for each $(x,y)\in\Omega$, acts as an upper bound on the loss $\ell(f_\theta(x+\delta),y)$ for any perturbed instance $x\mapsto x+\delta$.
\hh{have you defined $\Delta$ before?}

The optimization problem in~\eqref{eq:p-epi} offers an alternative view of the minimax problem in~\eqref{eq:p-rob}.  However, at first glance, it is not immediately clear how this problem can be used to generalize existing notions of robustness.  To this end, we now consider a \emph{stochastic} optimization problem which subsumes~\eqref{eq:p-epi} as a special case and naturally engenders interpretable, probabilisitic notions of intermediate robustness.  To this end, we assume that we are given a distribution $\Prob_\Delta$ over $\Delta$ and a confidence parameter $\beta\in[0,1]$.  We then consider the following problem, which will be a central object of study in this paper:
%
\begin{mdframed}[roundcorner=5pt, backgroundcolor=yellow!8]
\begin{alignat}{2}
    &\min_{\theta\in\Theta, \: t\in L^p} &&\E_{(x,y)} t(x,y) \tag{P-PROB} \label{eq:p-const} \\
    &\st &&\Prob_\Delta\left\{\ell(f_\theta(x+\delta), y) \leq t(x,y)\right\} \geq 1-\beta \notag
\end{alignat}
\end{mdframed}
%
where the constraint is enforced $\forall (x,y)\in\Omega$.   Notably, for $\beta=0$, we recover~\eqref{eq:p-rob} up to $\Prob_\Delta$-measure-zero sets, as the equality $\Prob_\Delta\{\ell(f_\theta(x+\delta), y) \leq t(x,y)\} = 1$ implies that $\ell(f_\theta(x+\delta), y) \leq t(x,y)$ for almost every $\delta\sim\Prob_\Delta$.   Moreover, for any $\beta > 0$, this problem is a relaxation of~\eqref{eq:p-epi} in the sense that the constraints are only required to hold with probability $1-\beta$ rather than for all $\delta\in\Delta$.  Thus, a smaller value of $\beta$ engenders a problem in which the constraint must hold with higher probability.


\paragraph{The special case of the 0-1 loss.}   
Let us assume that the loss function $\ell$ is the 0-1 loss, i.e.\ $\ell(f_\theta(x),y) = \mathbbm{1}\{f_\theta(x)\neq y\}$.  In this case, it is straightforward to show that~\eqref{eq:p-epi} is equivalent to an \emph{unconstrained} stochastic problem.
%
\begin{remark} \label{rmk:rob-01-loss}
Given $\beta\in[0,1]$ and a distribution $\Prob_\Delta$ over $\Delta$, it holds that~\eqref{eq:p-const} is equivalent to
%
\begin{align}
    \min_{\theta\in\Theta} \quad \mathbb{E}_{(x,y)} \left[ \mathbbm{1}\{\Prob_\Delta\{f(x+\delta)\neq y\} \geq \beta \} \right]. \label{eq:01-loss-unconst}
\end{align}
\end{remark}
%
Therefore, under the 0-1 loss, the problem in~\eqref{eq:p-const} can be rewritten in terms of a new loss function $\mathbbm{1}\{\Prob_\Delta\{f(x+\delta)\neq y\} \geq \beta \}$ that returns a loss value of one when the event $f_\theta(x+\delta)\neq y$ occurs with probability greater than $\beta$ over $\Prob_\Delta$, and zero otherwise.







==> old/intro.tex <==
\section{Introduction}

% Paragraph 1: THE STATE OF THINGS
% Learning is good, ERM works.  But ERM is bad also.  AT improves robustness, but is overly conservative, has fundamental trade-offs.


Due to its well-documented success in a variety of domains, learning has become an integral part of many modern information systems.   Underlying much of this success is a statistical paradigm known as empirical risk minimization (ERM), in which a predictor is trained by minimizing an averaged cost function.  And while ERM is now ubiquitous in practice, it has recently been shown that the complex prediction rules learned
by ERM suffer from a severe lack of robustness, which in turn greatly limits the applicability of these predictors to safety-critical domains.  Indeed, the pressing nature of this vulnerability has led to pronounced interest in improving the so-called adversarial robustness of modern learning tools.  

To meet this need, a growing body of work has motivated a new learning paradigm known as \emph{adversarial training}, wherein predictors are trained by minimizing a worst-case cost function, as opposed to the average-case paradigm employed by ERM.  And despite a great deal of empirical evidence which shows that adversarial training improves the robustness of learned predictors, this framework is not without its drawbacks.  Indeed, adversarial training is known to be highly conservative, which in turn engenders a fundamental trade-off between robustness and nominal performance.  Furthermore, the problem of computing the worst-case cost function is nonconvex and underparameterized for most modern learning models, including deep neural networks.  

% Paragraph 2: WHAT IS THE PROBLEM
% There is a need to reconcile these two objectives.  Avoid fundamental trade-offs, maintain high nominal accuracy, but still be robust to perturbations.  

% Paragraph 3: WHAT DO WE WANT IN A SOLUTION
% Fit average and worst case in the same principled framework, interpretable, ability to train.  

% \textcolor{red}{Nature doesn't act adversarially.}

To summarize, the fundamental drawbacks of existing learning paradigms motivate the need for a new framework for robust learning that avoids the conservatism and fundamental trade-offs of adversarial training while simultaneously maintaining high levels of robustness.  To this end, in this paper we propose a framework called \emph{probabilistic robustness} to bridge the gap between the accurate, yet brittle average case used in ERM and the robust, yet conservative worst case approach used in adversarial training.  Our key insight is that by enforcing robustness to most rather than to all perturbations, we can theoretically and empirically avoid the fundamental drawbacks of adversarial training while maintaining high levels of robustness as well as similar levels of nominal performance to predictors trained using ERM.  In particular, our contributions are as follows:
%
\begin{itemize}[nolistsep,leftmargin=1em]
    \item \textbf{New problem setting.}  We introduce a new problem setting which we call \emph{probabilistic robustness}, wherein the goal is to obtain predictors that are robust to most rather than to all perturbations.
    \item \textbf{Fundamental trade-offs.}  In two foundational settings, we study the trade-offs between probabilistic robustness and nominal performance at optimality; ultimately we show that unlike in adversarial robustness, there is no trade-off between probabilistic robustness and nominal performance in high dimensions.
    \item \textbf{Learning theoretic analysis.}
    \item \textbf{Tractable algorithm.}  By exploiting the connections between probabilistic robustness and risk-aware estimation, we propose a tractable algorithm for training probabilistically robust classifiers.
    \item \textbf{Experimental evaluation.}  We provide experiments on MNIST, CIFAR-10, and SVHN which show that our algorithm effectively enforces probabilistic robustness without trading off in nominal performance vis-a-vis ERM.
\end{itemize}




% \begin{itemize}
%     \item Our framework, (1) lies between average-case and worst-case, (2) does not suffer from fundamental trade-offs between robustness and accuracy, (3) is PAC learnable, (4) is interpretable, and (5) significantly improves robustness with respect to intermediate metrics of risk.  
% \end{itemize}

% \begin{itemize}
%     \item \textbf{New robustness framework.}  We introduce a principled framework for intermediate robustness between the average-case and worst-case.  Unlike past work, our main idea is to minimize a \emph{coherent}, interpretable risk metric.
%     \item \textbf{Trade-offs between robustness and accuracy.}  In a high-dimensional mixture-of-Gaussians setting, we show that there is no trade-off between our notion of robustness and nominal performance.  On the other hand, we show that in this setting there is a significant trade-off between adversarial robustness and nominal performance, which is consistent with past work.
%     \item \textbf{PAC learnability.}  In contrast to the setting of adversarial robustness, we show that our notion of robustness is PAC learnable, in the sense that is is possible to obtain a robust classifer from a polynomial number of samples.
%     \item \textbf{New algorithm.}  We propose a scalable primal-dual algorithm for training deep models to be robust in our framework.  Our algorithm significantly outperforms all baseline algorithms on a family of new robustness metrics, while simultaneously achieving the same nominal performance of ERM.
%     \item\textbf{Experiments} New metrics of risk, more natural for evaluating robustness
% \end{itemize}


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=0.7\columnwidth]{figs/erm.pdf}
        \caption{\textbf{Empirical risk minimization.}}
        \label{fig:erm}
    \end{subfigure}\quad
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=0.7\columnwidth]{figs/adv_rob.pdf}
        \caption{\textbf{Adversarial training.}}
        \label{fig:adv-rob}
    \end{subfigure}\quad
    \begin{subfigure}[b]{0.31\textwidth}
        \centering
        \includegraphics[width=0.7\textwidth]{figs/rrm.pdf}
        \caption{\textbf{Probabilistically Robust Training.}}
        \label{fig:rrm}
    \end{subfigure}
    \caption{Comparison between ERM, AT, and PRT.}
    \label{fig:comparison}
\end{figure*}


==> old/prelims.tex <==
\section{Existing robust learning paradigms}

In this paper, we consider a standard supervised learning setting in which the data is distributed according to an unknown joint distribution $\calD$ over instance-label pairs $(x,y)$, where the instances $x\in\calX$ are supported on a compact subset $\calX$ of $\R^d$ and that the labels $y\in\calY:=\{1,\dots,K\}$ take on integer values between 1 and $K$.  We let $(\Omega,\calB)$ denote the underlying measurable space, where $\Omega = \calX\times\calY$ denotes the data space and $\calB$ denotes the Borel $\sigma$-algebra over $\Omega$.  We also assume that the joint distribution $\calD$ admits a density $\Prob(x,y)$ defined over the Borel sets in $\calB$.  

Ultimately, our goal is to learn a classifier that can correctly predict the label $y$ of a corresponding instance $x$ whenever $(x,y)\sim\calD$.  In particular, we consider classifiers $f_\theta:\R^d\to\calS^K$ parameterized by a vector $\theta$ drawn from a compact set $\Theta\subset\R^p$, where $S^K$ denotes the $(K-1)$ simplex.  Further, we denote the hypothesis class of all classifiers by $\calH = \{f_\theta : \theta\in\Theta\}$.  In this way, we can think of each classifier as returning a $K$-dimensional vector $f_\theta(x)$ where each component $[f_\theta(x)]_k$ of the output denotes the probability that $y = k$.  Given such a classifier $f_\theta$ and an input instance $x$, we predict a label $\hat{y}(x)$ via the classification rule $\hat{y}(x) \in \argmax_{k\in\calY} \left[f_\theta(x)\right]_k$, where ties are broken arbitrarily.  To this end, the statistical problem of training a classifier to correctly predict the label $y$ of a corresponding instance $x$ drawn randomly from $\calD$ can be written as
%
\begin{prob}[\textup{P-NOM}]
    \min_{\theta\in\Theta} \: \E_{(x,y)} \left[\ell(f_\theta(x),y)\right] \label{eq:nom-training}
\end{prob}
%
where $\ell:\calY\times\calY\to\R_{\geq 0}$ is a suitably-chosen loss function (e.g.\ the cross-entropy or squared loss).  The ubiquitous ERM paradigm is a special case of~\eqref{eq:nom-training}, wherein the expectation in~\eqref{eq:nom-training} is replaced by its empirical counterpart over finitely-many instance-label pairs sampled i.i.d.\ from $\calD$ (see Figure~\ref{fig:erm}).

We assume that the map $(x,y)\mapsto\ell(f_\theta(x),y)$ is integrable so that the expectation $\E_{(x,y)}[ \ell(f_\theta(x),y)]$ in~\eqref{eq:nom-training} is well-defined, and that this map is an element of the Lebesgue space $L^p(\Omega, \calB, \Prob)$ for some $p\in(1,\infty)$.  

\paragraph{Standard formulations for robust learning.}    In recent years, there has been pronounced interest in improving the robustness of state-of-the-art classifiers to variation in the input data.  Indeed, for modern choices of hypothesis classes $\calH$ (e.g.\ the class of deep neural networks), a rapidly growing body of work has shown that classifiers learned via ERM are sensitive to imperceptible perturbations of data.   In other words, given an instance $x$ and a trained classifier $f_\theta$, one can often find a small perturbation $\delta$ such that $f_\theta(x)$ is correctly classified, whereas $f_\theta(x+\delta)$ is classified incorrectly.  In this setting, the perturbations $\delta$ are assumed to be drawn from a set $\Delta\subset\R^d$, where $\Delta$ is typically chosen to be a closed ball with respect to a given metric on Euclidean space, i.e., $\Delta = \{\delta\in\R^d : \norm{\delta}\leq \epsilon\}$.  However, we do not make any particular assumptions on the form of $\Delta$ in this paper, and indeed our results apply more generally to arbitrary perturbation sets, such as those considered in~\cite{goodfellow2009measuring,wong2020learning,robey2020model}.

As pointed out in~\cite{rice2021robustness}, the vast majority of the literature concerning the robustness of learning methods has focused on two disparate paradigms of robustness.  In the first paradigm, robustness is evaluated with respect to the expected cost over randomly generated perturbations to the input data.  Thus, given a distribution $\Prob_\Delta$ over perturbations $\delta\in\Delta$, training a classifier to be robust in this setting can be formulated as follows: 
%
\begin{prob}[\textup{P-AVG}]
    \min_{\theta\in\Theta} \: \E_{(x,y)} \left[ \E_{\delta\sim\Prob_\Delta} \left[ \ell(f_\theta(x+\delta),y) \right] \right]. \label{eq:p-avg}
\end{prob}
%
This notion of robustness underlies numerous algorithms, including various data augmentation methods~\cite{holmstrom1992using,van2001art,krizhevsky2012imagenet,volpi2018generalizing,hendrycks2019benchmarking,hendrycks2019augmix,chen2020group}.  

In the second paradigm, robustness is evaluated with respect to \emph{adversarially-chosen}, worst-case perturbations of data, which can be formulated as the following robust optimization problem:
%
\begin{prob}[\textup{P-ROB}]
    \min_{\theta\in\Theta} \: \E_{(x,y)} \left[\max_{\delta\in\Delta} \: \ell(f_\theta(x+\delta),y)\right] \label{eq:p-rob}
\end{prob}
%
In~\eqref{eq:p-rob}, solving the inner problem for a fixed instance $x$ amounts to finding a perturbation $\delta^\star\in\Delta$ such that $x+\delta^\star$ is most likely to be misclassified by the classifier $f_\theta$.  Numerous principled algorithms have been proposed for solving this problem~\cite{goodfellow2014explaining,madry2017towards,kannan2018adversarial,robey2021adversarial} as well as closely-related robust variants of this problem~\cite{biggio2013evasion,moosavi2016deepfool,wong2018provable,wang2019improving,zhang2019theoretically}.  

\paragraph{Drawbacks of existing robustness paradigms.}

Although the formulations in~\eqref{eq:p-avg} and~\eqref{eq:p-rob} have contributed to significant improvements in the robustness of state-of-the-art classifiers, both paradigms have notable drawbacks.  Indeed, while classifiers trained by solving the average-case robustness problem in~\eqref{eq:p-avg} typically achieve strong nominal performance, such classifiers are often severely lacking in robustness~\cite{szegedy2013intriguing}.  On the other hand, while classifiers trained via~\eqref{eq:p-rob} are significantly more robust to adversarially-generated perturbations, this improvement comes at the cost of a fundamental trade-off between robustness and nominal performance~\cite{tsipras2018robustness,dobriban2020provable,javanmard2020precise}.  Moreover, solving~\eqref{eq:p-rob} presents a significant challenge, as the inner maximization is nonconcave and severely underparameterized for many modern function classes (e.g.\ deep neural networks), leading to a highly non-favorable optimization landscape~\cite{soltanolkotabi2018theoretical}.  To summarize there is a significant gap between the accurate, yet brittle average-case notion of robustness in~\eqref{eq:p-avg} and the robust, yet conservative notion of robustness in~\eqref{eq:p-rob}.  


\paragraph{Interpolating between the average and worst case.}

Toward addressing this shortcoming of the standard robust learning paradigms in~\eqref{eq:p-avg} and~\eqref{eq:p-rob}, two recent works have sought to connect these paradigms with the goal of deriving an intermediate notion of robustness between the worst and average case.  In the first work, ~\cite{rice2021robustness}  observe that one can interpolate between~\eqref{eq:p-avg} and~\eqref{eq:p-rob} by treating the loss as the value of a particular functional norm.  More specifically, by letting $(\Delta, \calB_\Delta, \Prob_\Delta)$ be a measure space over the space of perturbations and by assuming that the loss is non-negative, one can view the following problem 
%
\begin{align}
    \min_{\theta\in\Theta} \: \mathbb{E}_{(x,y)}  \norm{\ell(f_\theta(x+\delta),y)}_{L^p(\Delta, \calB_\Delta, \Prob_\Delta)} \label{eq:rice}
\end{align}
%
as subsuming~\eqref{eq:p-avg} and~\eqref{eq:p-rob} as special cases for $p=1$ and $p=\infty$ respectively.  On the other hand, in~\cite{li2020tilted,li2021tilted}, the authors study the following problem
%
\begin{align}
    \min_{\theta\in\Theta} \: \E_{(x,y)} \left[\frac{1}{t} \log\left( \mathbb{E}_{\delta} \left[ e^{ t \cdot \ell(f_\theta(x+\delta),y)}  \right]\right) \right] \label{eq:term}
\end{align}
%
for which it holds that~\eqref{eq:p-avg} and~\eqref{eq:p-rob} can be recovered as $t\to 0$ and $t\to\infty$ respectively. 

While both of these proposed methods do interpolate between the average and worst case, they also suffer from significant drawbacks.  In the case of~\cite{rice2021robustness}, evaluating the functional norm of interest is prohibitively challenging; indeed, as acknowledged by the authors, it is not compuationally feasible to  accurately approximate the norm in~\eqref{eq:rice} during training.  In the case of~\cite{li2020tilted,li2021tilted}, training at either end of the range $(0,\infty)$ for $t$  can become unstable.  Furthermore, both~\eqref{eq:rice} and~\eqref{eq:term} lack interpretibility, as both interpolation schemes rely on somewhat nebulous parameters ($p$ and $t$ respectively)  which have no physically-interpretable meanings.


==> old/trade-offs.tex <==
\section{Fundamental trade-offs for probabilistic robustness} \label{sect:analysis}

In the setting of adversarial robustness, a significant body of work has studied the trade-offs between nominal performance and robustness.  Indeed, the consensus among many of these works is that adversarial robustness and nominal performance are fundamentally at odds~\cite{dobriban2020provable,dan2020sharp,javanmard2020precise}. And indeed, this view has also been corroborated in a variety of large-scale empirical studies~\cite{su2018robustness,tsipras2018robustness,zhang2019theoretically}.  In this way, to build intuition for the probabilistic robustness setting introduced in~\ref{eq:p-const}, we study our framework in two fundamental settings: binary classification and linear regression.

\subsection{Binary classification} \label{sect:bin-class}

We first consider a two-class Gaussian classification setting, in which the data is distributed as follows:
%
\begin{align} \label{eq:mix-of-gaussian}
    x|y \sim \mathcal{N}(y\mu, \sigma^2 I_d), \qquad y = \begin{cases}
        +1 &\:\text{w.p. } \pi \\
        -1 &\:\text{w.p. } 1-\pi.
    \end{cases}
\end{align}
%
In this setting, $\pi\in[0,1]$ is the proportion of the $y=+1$ class, $I_d$ denotes the $d$-dimensional identity matrix, $\sigma>0$ is the within-class standard deviation, and without loss of generality we assume that the means $\pm\mu$ are centered about the origin.  By scaling, we can also take $\sigma=1$.  Throughout this section, we let $\epsilon>0$ be given and we consider perturbation sets $\Delta = \{\delta\in\R^d : \norm{\delta}_2\leq \epsilon\}$ under the uniform distribution $\fkr$.  For notational convenience, we define the log-odds ratio as $q := \ln\{(1-\pi)/\pi\}$ and we define $\ln(0) := -\infty$ and $\sign(0):=1$.  

In this setting, it is well-known that the Bayes optimal classifier is $h^\star_\textup{Bayes}(x) = \sign(x^\top \mu - q/2)$~\cite{anderson1958introduction}.  Moreover,~\cite{dobriban2020provable} recently showed that the optimal adversarially robust classifier is $h^\star_\textup{rob}(x) = \sign( x^\top\mu(1 - \epsilon/\norm{\mu}_2)_+ - q/2)$.  To this end, in the following result we derive closed-form expressions for optimal probabilistically robust classifiers.
%
\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/spherical_cap.png}
    \caption{Spherical cap}
    \label{fig:spherical-cap}
\end{figure}
%
\begin{proposition} \label{prop:opt-beta-rob-gaussian}
Suppose that the data is distributed according to~\eqref{eq:mix-of-gaussian} and let $\epsilon>0$ be such that $\epsilon < \norm{\mu}_2$.  Then for any $\beta\in[0, 1/2]$, an optimal classifier for~\eqref{eq:p-const} is 
%
\begin{align}
    h^\star(x) =
        \sign\left(x^\top \mu\left(1 - \frac{h_\beta}{\norm{\mu}_2} \right)_+ - \frac{q}{2}\right). \label{eq:mix-gaussians-opt-classifier}
\end{align}
%
where $(z)_+ := \max\{0,z\}$ and $h_\beta$ is the Euclidean distance from the center of $\Delta$ to a spherical cap of $\Delta$ having volume $\beta$.  Moreover, it holds that
%
\begin{align}
    \PR(h^\star; \rho) - \SR(h^\star_\textup{Bayes}) = \begin{cases}
        O(\frac{1}{\sqrt{d}}) &\:\: \beta\in(0,\frac{1}{2}] \\
        O(1) &\:\: \beta = 0.
    \end{cases} \label{eq:mix-of-gauss-risk-diff}
\end{align} 
\end{proposition}
%
Concretely, this proposition conveys three key messages.  Firstly, we show the nontrivial fact that the optimal probabilistically robust classifier is \emph{linear}.  Indeed, the expression in~\eqref{eq:mix-gaussians-opt-classifier} corresponds to the Bayes optimal classifier with reduced effective mean $\mu\mapsto \mu(1-h_\beta/\norm{\mu}_2)_+$.  Secondly, the optimal probabilistically robust classifier depends directly on $\beta$ through the volume of a spherical cap of $\Delta$ (see Figure~\ref{fig:spherical-cap}).  It straightforward to check that as $h_{1/2} = 0$ and $h_0 = \epsilon$,~\eqref{eq:mix-gaussians-opt-classifier} subsumes $h^\star_\text{Bayes}$ and $h^\star_{\text{rob}}$ respectively as special cases.  Therefore, in this setting $\beta$ can be thought of as a tunable parameter that facilitates interpolation between the solutions to~\eqref{eq:nom-training} and~\eqref{eq:p-rob}.  And finally,~\eqref{eq:mix-of-gauss-risk-diff} tells us that the gap between the best achievable nominal performance and the best achievable probabilistic robustness vanishes in high dimensions for any $\beta > 0$.  Thus, as the dimension $d$ grows large, there is no trade-off between these two quantities.  On the other hand, when $\beta = 0$, there is a constant gap between these quantities, meaning that there is a non-trivial trade-off between adversarial robustness and nominal performance.

\subsection{Linear regression}

We next consider the setting of linear regression, wherein it is assumed that there exists an underlying parameter vector $\theta_0\in\Theta\subset\R^d$, and that the data is subsequently generated according to the following model:
%
\begin{align}
    x\sim\calN(0, I_d), \quad y = \theta_0^\top x + z, \quad z\sim\calN(0, \sigma^2) \label{eq:lin-reg-data}
\end{align}
%
where $\sigma>0$ is a fixed noise level.  Throughout, we let $\epsilon>0$ be given and we consider the perturbation set $\Delta = \{\delta\in\R^d : \norm{\delta}_2 \leq \epsilon\}$ under the uniform distribution $\fkr$.  Furthermore, we consider hypotheses of the form $f_\theta(x) = \theta^\top x$ for $\theta\in\Theta$, and we use the squared loss $\ell(f_\theta(x),y) = (f_\theta(x) - y)^2$.  In this setting, it is straightforward to calculate that at optimality $\SR(f_{\theta}) = \sigma^2$, which is achieved for~$\theta=\theta_0$.  Moreover, in the more general probabilistic robustness setting, we have the following complementary result:
%
\begin{proposition}
Suppose that the data is distributed according to~\eqref{eq:lin-reg-data}.  Let $\theta^\star\in\Theta$ denote the optimal solution obtained by solving~\eqref{eq:p-const} over $\Theta$.  Then for any $\rho > 0$,
%
\begin{align}
    \PR(f_{\theta^\star}; \rho) - \SR(f_{\theta_0}) = \begin{cases} 
        O(1/\sqrt{d}) &\: \beta > 0 \\
        O(1) &\: \beta = 0
    \end{cases}
\end{align}
\end{proposition}
%
In this way, as in the previous subsection, it holds that for any $\beta > 0$, the gap between probabilistic robustness and nominal performance vanishes in high dimensions.  On the other hand, as was recently shown in~\cite{javanmard2020precise}, there exists a non-trivial gap between adversarial robustness and clean accuracy that does not vanish to zero by increasing the dimension in this setting.

\subsection{Sample complexity}

\begin{proposition}
Consider the 0-1 loss function and a robust measure~$\fkr$ absolutely continuous with respect to the Lebesgue measure~(non-atomic). For any~$\rho^\prime > 0$, there exists a hypothesis class~$\calH^\prime$ such that the sample complexity of probabilistically robust learning with~$\rho < \rho^\prime$ is arbitrarily larger than that of~$\rho \geq \rho^\prime$. In particular, the latter is the same as the sample complexity of~\eqref{eq:nom-training}.
\end{proposition}

\begin{proof}
Let us begin by reducing the task of determining the sample complexity of these problems to that of determining the VC dimension of their objectives:

\begin{lemma}\label{T:sample_complexity}
	Consider the values of~\eqref{eq:nom-training} and~\eqref{eq:erm} when the loss~$\ell$ takes values in~$\{0,1\}$. The number of samples needed for~$\big\vert P^\star - \hat{P}^\star \big\vert \leq \epsilon$ with probability~$1-\delta$ is
	%
	\begin{equation*}
		C_1 \frac{d_\text{VC} + \log(1/\delta)}{\epsilon^2} \leq N \leq C_2 \frac{d_\text{VC} + \log(1/\delta)}{\epsilon^2}
			\text{,}
	\end{equation*}
	%
	for universal constants~$C_1,C_2$. The VC dimension~$d_\text{VC}$ is defined the largest~$d$ such that~$\Pi(d) = 2^d$ for the \emph{growth function}
	%
	\begin{equation*}
		\Pi(d) = \max_{\{(x_n,y_n)\} \subset (\calX \times \calY)^d}\ \abs{ \calS\big( \{(x_n,y_n)\} \big) }
	\end{equation*}
	%
	where~$\calS\big( \{(x_n,y_n)\} \big) = \big\{u \in \{0,1\}^m \mid \exists h \in \calH \ \text{such that}\ \allowbreak u_n = \ell\big( h(x_n), y_n \big) \big\}$.
\end{lemma}

We now proceed with the construction of the hypothesis class using a modified version of that in~\blue{[REF, Lemma~2]}. Fix~$m \in \setN$ and pick~$\{c_1,\dots,c_m\} \in \calX^m$ such that, for~$\Delta_i = c_i + \Delta$, it holds that~$\Delta_i \cap \Delta_j = \emptyset$ for~$i \neq j$. Within each~$\Delta_i$, define~$2^{m-1}$ disjoint sets~$\calA_{i}^b$ with~$\fkr(\calA_{i}^b) \leq \rho^\prime/m$ labeled with the binary digits~$b \in \{0,1\}^m$ whose~$i$-th digit is one. In other words, $\Delta_1$ contains sets with signature~$1 \mathsf{b}_2 \dots \mathsf{b}_m$ and~$\Delta_3$ contains sets with signature~$\mathsf{b}_1 \mathsf{b}_2 1 \dots \mathsf{b}_m$. Observe that there are indeed~$2^{m-1}$ sets~$\calA_{i}^b$ for each~$i$, that their signatures span all possible~$m$-digits binary numbers, and there are at most~$m$ sets with the same signature~(explicitly, for~$b = 11\dots1$). Also note that while each~$\calA_{i}^b$ may measure considerably less than~$\rho^\prime$, such sets always exist since~$\fkr$ is non-atomic.

We can now construct the hypothesis class~$\calH^\prime = \{h_b \mid b \in \{0,1\}^m\}$ by taking
%
\begin{equation}\label{eq:hypothesis}
	h_b(x) = \begin{cases}
		1 \text{,} &x \notin \bigcup_{i = 1}^m \calA_{i}^b
		\\
		0 \text{,} &x \in \bigcup_{i = 1}^m \calA_{i}^b
	\end{cases}
\end{equation}

Let us proceed first using the probabilistically robust loss~$\ell\big( h(x), y \big) = \rhosup_{\delta \sim \fkr}\ \indicator\big[ h(x+\delta) \neq y \big]$.

We begin by showing that if~$\rho < \rho^\prime$, then~$d_\text{VC} > m$. Indeed, consider the set of points~$\{(c_i,1)\}_{i=1,\dots,m} \subset (\calX \times \calY)^m$. In this case, the cardinality of~$\calS$ is exactly~$2^m$, i.e., this set can be shattered by~$\calH$. Indeed, for any signature~$b \in \{0,1\}^m$ and~$i = 1,\dots,m$, $\rhosup_{\delta \sim \fkr} \indicator[h_b(c_i + \delta) \neq 1] = b_i$. Using Lemma~\ref{T:sample_complexity}, we therefore conclude that~$N = \Theta\big( \log(\abs{\calH^\prime})/\epsilon^2 \big)$.

Let us now show that~$d_\text{VC} = 1$ for~$\rho \geq \rho^\prime$ by showing that~$\Pi(2) < 4$. To do so, we take two arbitrary points~$(x_1, y_1), (x_2, y_2) \in \calX \times \calY$ and proceed case-by-case. To simplify the exposition, define~$\calA = \cup_{i = 1}^m \cup_{b \in \{0,1\}^m} \calA_i^b$.

\begin{itemize}
	\item Suppose that~$(x_1 + \Delta) \cap \calA = \emptyset$. Then, observe from~\eqref{eq:hypothesis} that~$h(x_1 + \delta) = 1$ for all~$h \in \calH$ and~$\delta \in \Delta$. Hence, for all~$h \in \calH$, we obtain
	%
	\begin{equation*}
		\rhosup_{\delta \sim \fkr}\ \indicator\big[ h(x_1+\delta) \neq y_1 \big] = \indicator\big[ 1 \neq y_1 \big]
			\text{.}
	\end{equation*}
	%
	Depending on the value of~$y_1$, $\calS$ can only contain sets of the form~$(0,q)$ or~$(1,q)$, for~$q = \{0,1\}$. For such points, we therefore have~$\abs{\calS} \leq 2 < 4$. The same argument holds for~$x_2$.

	\item Suppose then that both~$(x_1 + \Delta) \cap \calA \neq \emptyset$ and~$(x_2 + \Delta) \cap \calA \neq \emptyset$. Then, $(x_j + \Delta)$ can intersect at most~$m$ sets~$\calA_{i}^b$ with the same signature~$b$~(explicitly, $b = 11\dots1$). But, by construction, $\fkr(\calA_i^b) \leq \rho^\prime/m$, which implies that~$\fkr(\cup_i \calA_i^{11\dots}) \leq \rho^\prime$. We then consider the possible labels separately:
	%
	\begin{itemize}
		\item for~$y_j = 1$, we know from~\eqref{eq:hypothesis} that~$\indicator\big[ h(x_j+\delta) \neq 1 \big] = 1$ only when~$x_j+\delta \in \calA_i^b$. But since~$\rho \geq \rho^\prime$, these sets can be ignored when computing the~$\rhosup$ and we get that for all~$h \in \calH$,
		%
		\begin{equation*}
			\rhosup_{\delta \sim \fkr}\ \indicator\big[ h(x_j+\delta) \neq 1 \big] = 0
				\text{;}
		\end{equation*}

		\item for~$y_j = 0$, we obtain from~\eqref{eq:hypothesis} that~$\indicator\big[ h_b(x_1+\delta) \neq 0 \big] = 1$ everywhere except when~$x_j+\delta \in \calA_i^b$. Hence, we obtain that for all~$h \in \calH$
		%
		\begin{equation*}
			\rhosup_{\delta \sim \fkr}\ \indicator\big[ h(x_j+\delta) \neq 1 \big] = q
				\text{.}
		\end{equation*}
		%
		where~$q = 0$ for large enough~$\rho$ or~$1$ otherwise. Either way, the value of the~$\rhosup$ does not depend on the hypothesis~$h$.
	\end{itemize}
	%
	Since the~$\rhosup$ does not vary over~$\calH$ for either~$x_1$ or~$x_2$, we conclude that~$\abs{\calS} \leq 2 < 4$, i.e., $\calH$ cannot shatter these points.
\end{itemize}
%
This implies~$d_\text{VC} \leq 1$ and since~$\abs{\calH} > 1$, we obtain~$d_\text{VC} = 1$. Using Lemma~\ref{T:sample_complexity}, we therefore conclude that~$N = \Theta\big( 1/\epsilon^2 \big)$.

Finally, we consider the case of~\eqref{eq:nom-training} for the nominal loss~$\ell\big( h(x), y \big) = \indicator\big[ h(x) \neq y \big]$. Once again, we take two points~$(x_1, y_1), (x_2, y_2) \in \calX \times \calY$ and proceed case-by-case.

\begin{itemize}
	\item Suppose, without loss of generality, that~$x_1 \notin \calA$. Then, \eqref{eq:hypothesis} yields~$h(x_1) = 1$ for all~$h \in \calH$ and~$\ell\big( h(x_1), y_1 \big) = \indicator\big[ 1 \neq y_1 \big]$. Depending on the value of~$y_1$, $\calS$ only has sets of the form~$(0,q)$ or~$(1,q)$, $q = \{0,1\}$. For such points, $\abs{\calS} \leq 2 < 4$. The same holds for~$x_2$.

	\item Suppose now that~$x_1 \in \calA_{i}^{b_1}$ and~$x_2 \in \calA_{i}^{b_2}$. Then, $h_b(x_j) = 0$ for~$b = b_j$ or~$h_b(x_j) = 1$ for~$b \neq b_j$. Hence,
	%
	\begin{itemize}
		\item if~$b_1 = b_2$, then~$h_b(x_1) = h_b(x_2)$. Depending on the value of the labels, $\calS$ only has sets of the form~$(q,q)$ or~$(1-q,q)$, $q = \{0,1\}$. For such points, we once again have~$\abs{\calS} \leq 2 < 4$;

		\item if~$b_1 \neq b_2$, then~$h_b(x_1) = 1 - h_b(x_2)$. Depending on the value of the labels, $\calS$ has, once again, only sets of the form~$(q,q)$ or~$(1-q,q)$, $q = \{0,1\}$. Hence, $\abs{\calS} \leq 2 < 4$ for such points;
	\end{itemize}
	%
\end{itemize}

In none of these cases~$\calH$ is able to shatter these two points, meaning that~$d_\text{VC} \leq 1$. Since~$\abs{\calH} > 1$, it holds that~$d_\text{VC} = 1$ which is indeed the same value as for~$\rho \geq \rho^\prime$.
%
%\red{If~$(x_1 + \Delta) \cap \Delta_i = \emptyset$ for all~$i$, then~$x_1 \notin \calA_i^b$ for all~$i$ and~$b$. From~\eqref{eq:hypothesis}, we observe that~$h(x_1 + \delta) = 1$ for all~$h \in \calH$ and~$\delta \in \Delta$. Hence, $\rhosup_{\delta \sim \fkr}\ \indicator\big[ h(x_1+\delta) \neq y_1 \big] = \indicator\big[ 1 \neq y_1 \big]$ and depending on the value of~$y_1$, $\calS$ only has sets of the form~$(0,q)$ or~$(1,q)$, $q = \{0,1\}$. For such points, $\abs{\calS} \leq 2 < 4$. The same holds for~$x_2$.
%
%Consider now the case in which~$(x_1 + \Delta) \cap \Delta_i \neq \emptyset$ and~$(x_2 + \Delta) \cap \Delta_j \neq \emptyset$ for some~$i,j = 1,\dots,m$. Without loss of generality, let us consider~$x_1$~($x_2$ will follow similarly). Notice that~$(x_1 + \Delta)$ can intersect at most~$m$ sets~$\calA_{i}^b$ with the same signature~$b$~(explicitly, $b = 11\dots1$) and~$\fkr(\cup_i \calA_i^{11\dots}) \leq \rho^\prime$. Observe from~\eqref{eq:hypothesis} that~$\indicator\big[ h(x_1+\delta) \neq 1 \big] = 1$ only when~$x_1+\delta \in \calA_i^b$. But since~$\rho \geq \rho^\prime$, these sets can be ignored when computing the~$\rhosup$ and we obtain~$\rhosup_{\delta \sim \fkr}\ \indicator\big[ h(x_1+\delta) \neq 1 \big] = 0$.
%
%Similarly, we obtain that~$\indicator\big[ h(x_1+\delta) \neq 0 \big] = 1$ everywhere except when~$x_1+\delta \in \calA_i^b$. For large enough~$\rho$, $\rhosup_{\delta \sim \fkr}\ \indicator\big[ h(x_1+\delta) \neq 0 \big] = 0$ for all~$h \in \calH$. Otherwise, $\rhosup_{\delta \sim \fkr}\ \indicator\big[ h(x_1+\delta) \neq 0 \big] = 1$ for all~$h \in \calH$. Either way, the value of the~$\rhosup$ does not vary over~$\calH$ for either~$x_1$ or~$x_2$, concluding that~$\abs{\calS} \leq 2 < 4$, i.e., $\calH$ cannot shatter those points. This implies~$d_\text{VC} \leq 1$ and since~$\abs{\calH} > 1$, we obtain~$d_\text{VC} = 1$. Using Lemma~\ref{T:sample_complexity}, we therefore conclude that~$N = \Theta\big( 1/\epsilon^2 \big)$.
%
%The case of~\eqref{eq:nom-training} follows similarly. Indeed, let~$\ell\big( h(x), y \big) = \indicator\big[ h(x) \neq y \big]$ and take two points~$(x_1, y_1), (x_2, y_2) \in \calX \times \calY$. If~$x_1 \notin \cup_{i,b} \calA_{i}^b$, then~\eqref{eq:hypothesis} yields~$h(x_1) = 1$ for all~$h \in \calH$ and~$\ell\big( h(x_1), y_1 \big) = \indicator\big[ 1 \neq y_1 \big]$. Depending on the value of~$y_1$, $\calS$ only has sets of the form~$(0,q)$ or~$(1,q)$, $q = \{0,1\}$. For such points, $\abs{\calS} \leq 2 < 4$. The same holds for~$x_2$.
%
%Suppose then that~$x_1 \in \calA_{i}^{b_1}$ and~$x_2 \in \calA_{i}^{b_2}$. Then, $h_b(x_j) = 0$ for~$b = b_j$ or~$h_b(x_j) = 1$ for~$b \neq b_j$. So if~$b_1 = b_2$, then~$h_b(x_1) = h_b(x_2)$. Depending on the value of the labels, $\calS$ only has sets of the form~$(q,q)$ or~$(1-q,q)$, $q = \{0,1\}$. For such points, we once again have~$\abs{\calS} \leq 2 < 4$. On the other hand, if~$b_1 \neq b_2$, then~$h_b(x_1) = 1 - h_b(x_2)$. Depending on the value of the labels, $\calS$ has, once again, only sets of the form~$(q,q)$ or~$(1-q,q)$, $q = \{0,1\}$. In none of these cases~$\calH$ is able to shatter these two points, meaning that~$d_\text{VC} \leq 1$. Since~$\abs{\calH} > 1$, it holds that~$d_\text{VC} = 1$ which is indeed the same value as for~$\rho \geq \rho^\prime$.}
%
\end{proof}
